PAC Statistical Model Checking of Mean Payoff in Discrete- and Continuous-Time MDP

Markov decision processes (MDP) and continuous-time MDP (CTMDP) are the fundamental models for non-deterministic systems with probabilistic uncertainty. Mean payoff (a.k.a. long-run average reward) is one of the most classic objectives considered in their context. We provide the first algorithm to compute mean payoff probably approximately correctly in unknown MDP; further, we extend it to unknown CTMDP. We do not require any knowledge of the state space, only a lower bound on the minimum transition probability, which has been advocated in literature. In addition to providing probably approximately correct (PAC) bounds for our algorithm, we also demonstrate its practical nature by running experiments on standard benchmarks.

==> algo-backup.tex <==
DROP 2 PARA / MOVE TO INTRO
In this section, we describe our algorithm to learn mean-payoff strategies for blackbox MDPs with PAC guarantees.
As discussed in the previous section, we use Equation~\ref{eq:decomp} to compute the expected mean-payoff.
% However, this formula cannot be used directly in the blackbox model.
We need to compute the following for this purpose:
\begin{inparaenum}
\item the probability to reach the end-components under an optimal strategy
\item mean-payoff value of the end-components.
\end{inparaenum}
However, the difficulty in blackbox models is that we do not know the exact transition probabilities on the edges, or even the number of successors for an action from a state.
We need to estimate these quantities by visiting the state-action pairs multiple times, and thereby collecting samples.
A \emph{sample} here refers to the observation we make regarding the successor every time we visit a state-action pair.
% A \emph{sample} here refers to the number of times an action has been chosen from a state.
Our algorithm simulates the MDP by taking the most promising actions from every state, visits the states as they are encountered, and keeps augmenting the newly encountered states to a partial model.
We do several such simulations until we achieve a precise mean-payoff estimate.
%Given a precision on the mean-payoff value, and an error tolerance, our algorithm simulates the MDP starting from the initial state $\initstate$ by taking the most promising action from every state, visits the states as they are encountered, and keeps augmenting the newly encountered states to a partial model.
% Starting from $\initstate$, an \emph{episodic run} of the MDP is one that finishes when we visit a terminal state which is an element of the set $\{s_+, s_-, s_?\}$.
%We do several episodic runs before checking if the required precision on the mean-payoff has been achieved.
We note that our algorithm uses {\sf OnDemand Value Iteration}\cite{cav17}, and does not require an exhaustive exploration of the entire MDP.

The results of \cite{Chatterjee12} and \cite{Solan03} provide a method for estimating the number of times each state-action pair needs to be visited in an MDP to obtain a PAC bound on the expected mean-payoff value.
However, the required number of samples using these bounds is prohibitively large, and therefore, giving guarantees with such analysis is not feasible in practice.
%Our main contribution in this paper is to provide a practical algorithm which does not require us to construct the entire MDP model, but one can obtain an estimate of the expected mean-payoff from a partial model while providing PAC guarantees as described below.\todo{Do we talk about the \cite{atva} paper?}
Our main contribution in this paper is a practical algorithm that doesn't necessarily explore the entire MDP, while giving an estimate of the expected mean-payoff with PAC guarantees.

\paragraph*{Estimating transition probabilities}
In \cite{AKW19}, an analysis has been given to estimate bounds on transition probabilities for reachability objective in MDPs.
% We use the same analysis to find the number of samples required for estimating the bounds on the transition probabilities on paths reaching the end-components from the initial state.
We present the analysis here for completion.

Given an error tolerance $\delta$, we distribute the error tolerance over all individual transitions as $\delta_{\trans} := \dfrac{\delta\cdot \pmin}{\lvert\{{a} \vert\, \state \in \widehat{S} \wedge {a} \in \av(s) \}\rvert}$.
The quantity $\frac{1}{\pmin}$ gives an upper bound on the maximum number of possible successors for an available action from a state\footnote{If we know the maximum number of possible successors for some action over all states, we can use that too instead of $\frac{1}{\pmin}$ to obtain a slightly smaller confidence width. For example, in one of our benchmarks, zeroconf, we have $\pmin=0.002$, while the maximum number of successors over all state-actions pairs is $6$. Using maximum number of successors, we get a confidence width $c=0.0021$ as opposed to $0.0027$ when we use $\pmin$. A more detailed analysis is presented in Appendix~\ref{app:pminandmaxsuccessorcomparison}}.
%The Hoeffding's bound gives us a bound on the number of times an action $a$ needs to sampled from state $s$ ($\#(s,a)$) to achieve a confidence width $c \geqslant \sqrt{\dfrac{\ln \delta_\mathbb{T}}{-2\#(s, a)}}$.
The Hoeffding's inequality gives us a bound on the number of times an action $a$ needs to sampled from state $s$, denoted $\#(s,a)$, to achieve a confidence width $c \geqslant \sqrt{\dfrac{\ln \delta_\mathbb{T}}{-2\#(s, a)}}$ on $\trans(s,a,t)$, such that

%Now the lower bound of the probability on a transition from $s$ to a successor $t$ on action $a$ is computed as 
\begin{equation*}
\widehat{\mathbb{T}}(s,a,t) := \max (0, \dfrac{\#(s, a, t)}{\#(s, a)} - c)
\end{equation*}
where, $\#(s, a, t)$ is the number of times the $t$ is sampled when action $a$ is chosen from $s$.
\paragraph{Updating mean-payoff values}\todo{Redo after Section 3: expect $L(t)$ and $U(t)$ are defined there.}
Using $\widehat{\mathbb{T}}(s,a,t)$, we compute estimates of the upper and lower bounds of the values corresponding to every action from a state visited in the partial model that is constructed so far.
We denote these values using $\lb$ and $\ub$, such that $\lb(s)$ is a lower bound on the value of $s$.
% We obtain the following Bellman equation which is used to obtain an upper and a lower bound on the mean-payoff values for the blackbox setting.
We use the following \emph{modified} Bellman equations~\cite{AKW19}:

\begin{equation*}
\widehat{\lb}(s,a) := \sum\limits_{t:\#(s,a,t)>0} \widehat{\mathbb{T}}(s,a,t) \cdot \lb(t)
\end{equation*}
\begin{equation*}
\widehat{\ub}(s,a) := \sum\limits_{t:\#(s,a,t)>0} \widehat{\mathbb{T}}(s,a,t) \cdot \ub(t) + (1-\sum\limits_{t:\#(s,a,t)>0} \widehat{\mathbb{T}}(s,a,t)),
\end{equation*}
where $\lb(t) = \max\limits_{{a} \in \Av(t)} \widehat{\lb}(s,a)$ and $\ub(t) = \max\limits_{{a} \in \Av(t)}\widehat{\ub}(s,a)$.
When a state is discovered for the first time during the simulation, and is added to the partial model, we initialize $\lb(s)$, and $\ub(s)$ to 0, and 1, respectively.
Note that $\sum\limits_{t:\#(s,a,t) > 0} \widehat{\mathbb{T}}(s,a,t) < 1$. We attribute this remaining probability to unseen successors and assume their value to be 0 (1) to safely under (over)-approximate the lower (upper) bounds.
%The second term appears in the upper bound as a safe over-approximation of $1$ as the upper values of the target states \todo{can we call this `potential successors'?} not visited yet during taking action $a$ from state $s$. 
% \track{Add greybox update equations.}
We call these \emph{blackbox Bellman update} equations, since it assumes that all the successors of state $s$ have been not visited.
\paragraph*{Estimating values of end-components}
% In \cite{AKW19}, estimating values of end-components was not necessary since it deals with reachability objective.
% However, one would require to identify the end-components even for reachability objective so that an action leading outside the end-component can be taken to ensure that the simulation does not get stuck inside the end component.
The first step in estimating the value of end-components in an MDP is to find the end-components.
End-components are identified with an error tolerance of $\delta_{\trans}$.
Assuming an action has been sampled $n$ times, the probability of missing a transition for that action is at most $(1-\pmin)^n$.
Thus, we set $\delta_{\trans} \leqslant (1-\pmin)^n$ which gives us $n \geqslant \frac{\ln \delta_{\trans}}{\ln (1-\pmin)}$, i.e., for identifying ($T,A$) as a $\deltasure$ MEC, every action in $A$ that is available from a state $s \in T$ needs to be sampled at least $\frac{\ln \delta_{\trans}}{\ln (1-\pmin)}$ times.

Once a $\deltasure$ MEC $M$ is identified, we estimate its upper ($\gain^u_M$) and lower ($\gain^l_M$) bounds using value iteration.\footnote{Note that one requires the ECs to be aperiodic for the VI to converge.
We do \emph{not} add edges explicitly to the MEC, but we simulate the effect by using a hypothetical self-loop transition for every available action from each state with probability $(1-y)$, while the probabilities on the transitions to other states are multiplied by $y$ during the computation of the update equation~\cite{Puterman}.
An example illustrating this has been provided in Appendix~\ref{app:aperiodicity}.}
While running value iteration, we assume, with sufficient confidence, i.e., a small error tolerance, that there are no outgoing transitions.
So we use the following modified Bellman update equations inside the MEC in order to estimate the lower and the upper mean-payoff values, respectively.

% While running value iteration, we assume that the given set of states is indeed an MEC since it has been identified as a $\deltasure$ MEC, and with sufficient confidence, that is, a small error tolerance, we have that there are no outgoing transitions.
% So we use the following Bellman update equations inside the MEC in order to compute the upper and the lower mean-payoff values.
\begin{equation*}
\widehat{\lb}(s,a) := \sum\limits_{t:\#(s, a, t)>0} \widehat{\mathbb{T}}(s, a, t) \cdot \lb(t) + \min\limits_{t:\#(s, a, t)>0}\lb(t) \cdot (1-\sum\limits_{t:\#(s, a, t)>0} \widehat{\mathbb{T}}(s, a, t))
\end{equation*}
\begin{equation*}
\widehat{\ub}(s, a) := \sum\limits_{t:\#(s, a, t)>0} \widehat{\mathbb{T}}(s, a, t) \cdot \ub(t) + \max\limits_{t:\#(s, a, t)>0}\ub(t) \cdot (1-\sum\limits_{t:\#(s, a, t)>0} \widehat{\mathbb{T}}(s, a, t))
\end{equation*}
Under the assumption that all the successors from a state $s$ corresponding to an action $a$ have been visited, we under-(over-)approximate the lower(upper) bound to a much lesser degree. Following the assumption, we call these \emph{greybox} Bellman update equations. 

The value iteration algorithm further gives us bounds on $\gain^u_M$ and $\gain^l_M$. We say that the upper estimate of $\gain^u_M$ and the lower estimate of $\gain^l_M$ are the overall upper and lower bounds of the mean-payoff value of $M$. Now, in order to get convergence on the overall bounds, we need value iteration to return more precise estimates of $\gain^l$ and $\gain^u$, and we need to sample the actions inside $M$ many times to reduce the difference between $\gain^l$ and $\gain^u$. 
We call this procedure, $\mathsf{UPDATE\_MEC\_VALUE}$\footnote{This is outlined in detail in Appendix~\ref{app:algo}}.

Now, some MECs might have very low values or may not be reachable from the initial state with high probability. In such cases, no optimal strategy might visit these MECs, and it might not be efficient to obtain very precise mean-payoff values for every MEC that may be identified in an MDP. We follow an On-Demand heuristic\todo{Should be defined in Overview Section.} \cite{cav17} where we progressively increase the precision on mean-payoff values as an MEC seems more likely to be a part of an optimal strategy. The {\sf stay} action on MECs helps in guiding simulation towards those MECs that have a higher lower bound of the mean-payoff value. In particular, whenever the simulation ends up in $s_+$ or $s_?$, we run $\mathsf{UPDATE\_MEC\_VALUE}$ with higher precision on the MEC that led to these states. If the simulation ends up in these states through a particular MEC more often, it indicates that the lower bound of its mean-payoff value is reasonably high, and it would be worth increasing the precision on its mean-payoff value.
% Thus for computing the lower bound, we associate the remaining probability of $(1-\sum\limits_{t:\#(s, a, t)>0} \widehat{\mathbb{T}}(s, a, t))$ with the successor having the minimum value, while for computing the upper bound, we associate the remaining probability with the successor having the maximum value.
% As one can see, that these new set of Bellman update equations under-(over-) approximate the lower (upper) bound to a much lesser degree than the first type of Bellman equations.
% In these \emph{second type} of equations, we assume that all the successors of a state for an action have been visited, and hence we also call them \emph{greybox} Bellman update equations.
% This is \emph{not} required in blackbox learning for reachability objective~\cite{AKW19}.
% Since we want the confidence width on the value to be small to achieve the required input precision $\beta$ on the value, we need to sample the actions many times to achieve a small confidence width, and thereby obtain the required precision.
% If we find an MEC multiple times during the simulations, then it indicates that the MEC is easily reachable and has a greater effect on the mean-payoff of the MDP.
% We perform simulation and do increasingly more value iterations\footnote{Note that one requires the ECs to be aperiodic for the VI to converge.
% We do \emph{not} add edges explicitly to the MEC, but we simulate the effect by using a hypothetical self-loop transition for every available action from each state with probability $(1-y)$, while the probabilities on the transitions to other states are multiplied by $y$ during the computation of the update equation~\cite{Puterman}.
% An example illustrating this has been provided in Appendix~\ref{app:aperiodicity}.} on an MEC as it is visited more and more often to get more precision on its value.
% \track{Highlight that we do not seek precise values from the very beginning, but we do it successively.}
\begin{comment}
\paragraph{Simulation of MEC and VI inside MEC}
If we find an MEC multiple times during the simulations, then it indicates that the MEC is easily reachable and has a greater effect on the mean-payoff of the MDP.
% 
To achieve the target precision for the mean-payoff values, we need to have low confidence width on the probabilities of the transitions, particularly inside the MECs which also allows us to estimate the mean-payoff value of the MEC more precisely.
% Usually, the required precision for the mean-payoff values is several orders lower than the precision achieved during the course of the algorithm (the confidence width). To achieve the required precision, we need lower confidence width for the actions inside MECs. 
% We achieve this by simulating more `important' MECs a higher number times.
We perform simulation and do increasingly more value iterations on an MEC as it is visited more and more often to get more precision on its value.
% When we simulate an MEC for the first time, we simulate it to collect several 
\end{comment}
% $10000$ times the number of transitions in the MEC, that is, we visit a total of these many number of state-action pairs inside the MEC.
% In every subsequent visit of the same MEC, we multiply the number of samples to be collected by $5$ times. 
% The details can be found in Algorithm~\ref{alg:computeNSamples} in Appendix~\ref{app:algo}.
% For many of our benchmarks, the precision is met, while for the rest, we use a timeout of $30$ minutes and note the upper and the lower values.
% We would like to note that we used several benchmarks used in \cite{AKW19}, and we made several observations leading to optimizations so that the convergence rate is similar to the case of reachability objective reported in \cite{AKW19}.\todo{Check this entire paragraph with Chaitanya and Pazhamalai.}
\paragraph{Overall Algorithm and Details}
The overall on-demand value iteration algorithm has been outlined in Algorithm~\ref{alg:general}.
It takes as input an MDP $\Mdp$, a precision $\beta$ on the mean-payoff value, an error tolerance $\delta$, the maximum reward $\rmax$ over all transitions, and $\pmin$.
% and the sequence of number of simulations.
% \todo{What is the last parameter? Do we use this?: Are you talking about $p_{min}$? We do use it}.
% Further, the availability of the maximum number of successors may reduce the confidence width used on the transitions, particularly when the size of the MDP is small.
The upper and the lower values for $s_+$ are initialized to $1$, for $s_-$ to $0$, and for $s_?$. 
In Line~\ref{Ni}, $\mathcal{N}_i$ denotes the number of episodic runs we do during iteration $i$. An episodic run starts from $\initstate$, goes through the MDP, until it ends in a terminal state ($\{s_+, s_-,s_?\}$ in our case). We run multiple episodic runs to accumulate many samples before constructing the partial model.

% \track{Discuss $\mathcal{N}_i$.}
The $\SIMULATE$ function (detailed in Algorithm~\ref{alg:simulateNewMDP} in Appendix~\ref{app:algo}) performs an episodic run and ends when it reaches a terminal state, that is $s_+, s_?$, or $s_-$.
% During the run, the function identifies $\deltasure$ MECs and stores the path in a variable $w$.
Recall that a terminal state is reached from an MEC only through the {\sf stay} action.
If some state is visited some $k$ times during the run, this indicates a possible presence of an MEC, and hence we check for the existence of a $\deltasure$ MEC. In Lines~\ref{pop}-\ref{update_mec} of Algorithm~\ref{alg:general}, we check if an episodic run ends in $s_+$ or $s_?$, and in such case, we update the MEC value with increased precision.
%odels, and found faster convergence for them compared to results reported in~\cite{cav17}}.
% , not only for blackbox models, but also for the whitebox case studied in~\cite{cav17}.
Here $M$ is the MEC to which $q$ belongs, and $\gain^u_M-\gain^l_M$ indicates the current precision on the mean-payoff value of $M$. We run $\mathsf{UPDATE\_MEC\_VALUE}$ to reduce this difference and thereby increase the precision on the mean-payoff value.

\begin{algorithm}[tbp]
    \caption{Blackbox mean-payoff learning for MDPs}\label{alg:general}
    \hspace*{\algorithmicindent}\algorithmicrequire MDP $\Mdp$, precision $\beta > 0$, error tolerance $\delta > 0$, max weight $r_{max}$, revisit threshold $k \ge 2$, transition probability lower bound $\pmin$.\\
    % , number of simulations for every $i$, $\mathcal{N}_i$\. \\
    \hspace*{\algorithmicindent}\algorithmicensure upper and lower bound of mean-payoff estimate for $\Mdp$ that is $\beta$-close to the actual value with probability at least $1-\delta$.
    \begin{algorithmic}[1]
        \Procedure{$\mathsf{ON\_DEMAND\_BVI}$}{}
            \State Initialize values of $s_+, s_-, s_?$
            \State $i$ = 1, ${\states}^\prime = \emptyset$
            \Repeat
            % \State $i = 2\cdot i$  
            \For{$\mathcal{N}_i$ times} \label{Ni}
                \State $\fpath \gets \SIMULATE$ \Comment{$\fpath$ is the explored path}
                \State ${\states}^\prime \leftarrow {\states}^\prime \cup w$
                \State $\delta_{\trans} \gets \dfrac{\delta\cdot \pmin}{\lvert\{{a} \vert\, s \in {\states}^\prime \wedge {a} \in {\av}^\prime(s) \}\rvert}$
                \If{$\pop(\fpath) \in \{s_?, s_+\}$} \label{pop}
                    \State $q \gets \topx(\fpath)$
                    \State $\mathsf{UPDATE\_MEC\_VALUE}$($M, (\gain^u_M-\gain^l_M)/2$) 
                    \label{update_mec}
                    \State Update ${\trans}^\prime(s, \mathsf{stay})$ according to Definition 5
                \EndIf
            \EndFor
            \State $\mathsf{FIND\_MECS}$  \Comment{This in turn calls $\delta_{\mathbb{T}}$-sure EC.} \label{find_mec}
            \State $\INITIALIZE$ \label{initialize}
            \Repeat     %\Comment{In the current implementation, we run the loop until there is no significant change (fixed in code: $10^{-8}$) in neither of $\lb$ or $\ub$.}
                \State $\UPDATE({\states}^\prime)$  %\track{Does not match with function type.}
                \For{ $T \in $ MECS(${\states}^\prime$)}
                    \State $\mathsf{DEFLATE}(T)$
                \EndFor
            \Until{No change in $\lb$, $\ub$ for all states, respectively}
            \State Increment $i$
            \Until{$\ub(\initstate)$ - $\lb(\initstate) < \frac{2\beta}{r_{max}}$} \Comment{\track{Change to footnote.}Note that $\beta$ is an absolute precision value, and hence for larger $r_{max}$, to ensure the same difference between the upper and the lower values as compared to a smaller value of $r_{max}$, we would need more iterations.}
        \EndProcedure
    \end{algorithmic}
\end{algorithm}
Once simulation is done, new MECs might have been discovered and old MECs might have been discarded. We keep track of this information in Line~\ref{find_mec}. Such changes can have cascading effects on the values of all states, and they are thus, reset and recomputed.
We repeat this overall process until convergence or a specified timeout.
% After every such sequence of episodic runs, we check whether the precision is satisfied. If the precision is met, then we terminate. 
% Else we perform another sequence of episodic runs. 
% During every episodic run, we check for the existence of $\deltasure$ MECs in the partial model. 
\paragraph{Deflate operation}
Unlike in the case of computation of mean-payoff for whitebox models~\cite{AKW19} where an MEC is collapsed following the computation of its value, for blackbox learning, once a set states is identified as a $\deltasure$ MEC, we cannot collapse them \todo{revise once stay-augmented MECs are properly defined} as mentioned earlier while defining {\sf stay}-augmented MEC.
Recall that an action with higher upper value is chosen more frequently.
However, this may also result in \emph{not} exploring the actions outside the MEC since an action that returns the highest upper value may visit only states inside the MEC.
Hence we perform a \enquote{deflate} operation \cite{KKKW18} that sets the value of the MEC to the best outgoing action from the MEC, and we continue the simulation outside the MEC by taking this best outgoing action.
Note that one of the outgoing action is also the {\sf stay} action which reflects the value of the MEC itself.

The details of various procedures of our algorithm are given in Appendix~\ref{app:algo}.

\paragraph{Statistical guarantees}
We show here that Algorithm~\ref{alg:general} gives a PAC guarantee on learning mean-payoff values on an input blackbox MDP.
\begin{theorem}\label{thm:algo}
% Given an error tolerance $\delta$, for blackbox MDPs, Algorithm~\ref{alg:general} is an anytime algorithm such that whenever it is stopped, the returned upper and lower bounds of the mean-payoff estimate are PAC with probability $1-\delta$.
Algorithm~\ref{alg:general} is an anytime algorithm with the property that when it is stopped, it returns an interval for the mean-payoff value of the MDP that is PAC for the given error tolerance $\delta$.
\end{theorem}
The proof of this theorem appears in Appendix~\ref{app:mdp_proof}.
% \todo{Add description about deflate operation.: Might be best to simply cite KKKW'18.}
% \todo{Add description of the Heuristic simulation.}

\begin{comment}

% \begin{algorithm}[H]
% \caption{Simulation algorithm counting occurrences}\label{alg:simulateNewMDP}
% 		\hspace*{\algorithmicindent}\algorithmicrequire	MDP $\Mdp$, revisit threshold $k$.\\
% 		\hspace*{\algorithmicindent}\algorithmicensure Simulated path $X$
% \begin{algorithmic}[1]
% \Procedure{$\SIMULATE$}{}
%     \State $X \gets \emptyset$ \Comment{Stack of states visited during this simulation}
%     \State $\state \gets \initstate$ 
%     \Repeat
%     	\State $X \gets X \cup \state$ \Comment{Push $\state$ to $X$}
%     	\State ${\action} \gets $ sampled according to best$_{\ub, \lb}(\state)$
%     	\State $\highlight{\tsucc} \gets$ sampled according to $\trans(\state,{\action})$
%     	\State $\highlight{\text{Increment }\#(\state,{\action},\tsucc)}$
%     	\State $\state \gets \highlight{\tsucc}$
%         \If {$\mathsf{Appear}(X, \state) \ge k$}
%             \If{$\STUCK(X, \state)$}
%                 \State ${\action} = $ $\mathsf{BEST\_LEAVING\_ACTION}(T)$ \Comment{$T$ is the MEC to which $\state$ belongs; actions are ranked according to best$_{\ub, \lb}(\state)$}
%                 \State $\state$ = origin of ${\action}$
%             	\State $\tsucc \gets$ sampled according to $\trans(\state,{\action})$
%             	\State $\text{Increment }\#(\state,{\action},\tsucc)$
%             	\State $\state \gets \tsucc$
%             \EndIf
%         \EndIf
%     \Until{$\state \in \{s_+, s_-, s_?\}$}
%     \State \textbf{return} $X \cup \set{\state}$
% \EndProcedure
% \end{algorithmic}
% \end{algorithm}


% \begin{algorithm}[htbp]
% 	\caption{Check if we are probably looping and should stop the~simulation}\label{alg:stuck}
% 			\hspace*{\algorithmicindent}\algorithmicrequire	State set $X$, state $s$.\\
% 			\hspace*{\algorithmicindent}\algorithmicensure Boolean value (Yes/No).	
% 	\begin{algorithmic}[1]
% 		\Procedure{$\STUCK$}{State set $X$, state $\state$}
% 		\State \textbf{return } 
% 		$\highlight{\exists T \subseteq X \text{ s.t. } T \text{ is EC in partial model} \wedge \state \in T \wedge \SUREEC(T)}$
% 		\EndProcedure
% 	\end{algorithmic}
% \end{algorithm}


% \begin{algorithm}[htbp]
% 	\caption{Check whether we are $\deltasure$ that $T$ is an EC}\label{alg:sureEC}
% 			\hspace*{\algorithmicindent}\algorithmicrequire	State set $T$, $\delta_T$.\\
% 			\hspace*{\algorithmicindent}\algorithmicensure Boolean value (Yes/No).	
% 	\begin{algorithmic}[1]
% 		\Procedure{$\highlight{\SUREEC}$}{State set $T$}
% 		\State $\stepsUntilSure = \frac{\ln(\transdelta)}{\ln(1-p_{\min})}$
% 		\State $B \gets \set{(\state,{\action}) \mid \state \in T \wedge \neg (\state,{\action}) \leaves T}$ \Comment{Set of staying state-action pairs}
% 		\If{$\bigwedge_{(\state,{\action}) \in B} \#(\state,{\action}) > \stepsUntilSure$}
% 		    \State \textbf{return} True
% 		\Else 
% 		    \State \textbf{return} False
% 		\EndIf
% 		\EndProcedure
% 	\end{algorithmic}
% \end{algorithm}


% \begin{algorithm}[H]
% 	\caption{Algorithm to update MEC reward value and stay action}\label{alg:updateMEC}
% 		\hspace*{\algorithmicindent}\algorithmicrequire	$\delta_T$-sure EC $M_i=(T_i, A_i)$, required precision $\alpha$.
% 	\begin{algorithmic}[1]
% 	\Procedure{$\mathsf{UPDATE\_MEC\_VALUE}$}{$M_i, \alpha$} 
% 	    \State $nSamples = \mathsf{COMPUTE\_N\_SAMPLES}(M_i)$
	    
% 	    \State $\simulateMecStandard (M_i, nSamples)$
% 		\State ${\lb}_r(M_i), {\ub}_r(M_i) = \mathsf{VALUE\_ITERATION} (M_i, \alpha)$
% 		\State Update $\mathsf{stay}$ action according to Definition~\ref{def:bquo}.  %\track{Does updating the $\mathsf{stay}$ action also include adding it for the first time?}
% 	\State \Return ${\lb}_r(M_i), {\ub}_r(M_i)$
%     \EndProcedure
% 	\end{algorithmic}
% \end{algorithm}


% \begin{algorithm}[H]
% 	\caption{Algorithm that gives nSamples based on MEC}\label{alg:computeNSamples}
% 		\hspace*{\algorithmicindent}\algorithmicrequire	$\delta_T$-sure EC $M_i=(T_i, A_i)$.
% 	\begin{algorithmic}[1]
% 	\Procedure{$\mathsf{COMPUTE\_N\_SAMPLES}$}{$M_i$}
% 	    \State $leastVisitCount \gets \min\{\#(\state, \action) \mid \state \in T_i, \action \in A_i\} $
	    
% 	    \State $initialSamples \gets 10^4$
% 	    \State $mFactor \gets 5$
% 	    \State $nSamples \gets initialSamples$
	    
% 	    \While{$nSamples < leastVisitCount$}
% 	        \State $nSamples = nSamples * mFactor$
	        
% 	        \If{$nSamples > 10^8$}
% 	            \State $nSamples = 10^8$
% 	            \State $break$
% 	        \EndIf
% 	    \EndWhile
%     \EndProcedure
% 	\end{algorithmic}
% \end{algorithm}


% \begin{algorithm}[H]
% \caption{Simulation algorithm for MDP MEC}\label{alg:simulate_MEC_MDP}
% 		\hspace*{\algorithmicindent}\algorithmicrequire	MDP MEC $(T, A)$, $nSamples$.\\
% 		\hspace*{\algorithmicindent}\algorithmicensure estimated transition probabilities for state-action pairs.
% \begin{algorithmic}[1]
% \Procedure{$\simulateMecStandard ()$}{}
%     \State $\state \gets \initstate$
%     \While{$\exists (\state, \action) \in T_i \times \av(\state) \text{ s.t. } \#(\state, \action) < nSamples$}
%     	\State ${\action} \gets $ sampled uniformly from $\state$
%     	\State $\highlight{\tsucc} \gets$ sampled according to $\trans(\state,{\action})$
%     	\State $\highlight{\text{Increment }\#(\state,{\action},\tsucc)}$
%     	\State $\state \gets \highlight{\tsucc}$ \Comment{Move from $s$ to $t$.}
%     \EndWhile
% \EndProcedure
% \end{algorithmic}
% \end{algorithm}

% \begin{algorithm}[H]
% \caption{Simulation algorithm for MDP MEC}\label{alg:simulate_MEC_MDP_CHEAT}
% 		\hspace*{\algorithmicindent}\algorithmicrequire	MDP MEC $(T, A)$, $nSamples$.\\
% 		\hspace*{\algorithmicindent}\algorithmicensure estimated transition probabilities for state-action pairs.
% \begin{algorithmic}[1]
% \Procedure{$\simulateMecDirAccess ()$}{}
%     \For{${\action}_i \in A_i$}
%       \For{$nSamples$ times}
%         \State Simulate ${\action}_i$ and update counts
%       \EndFor
%     \EndFor
% \EndProcedure
% \end{algorithmic}
% \end{algorithm}


% \begin{algorithm}[H]
% \caption{Simulation algorithm for MDP MEC}\label{alg:simulate_MEC_MDP_HEURISTIC}
% 		\hspace*{\algorithmicindent}\algorithmicrequire	MDP MEC $(T, A)$, $nSamples$, $nTransitions$.\\
% 		\hspace*{\algorithmicindent}\algorithmicensure estimated transition probabilities for state-action pairs.
% \begin{algorithmic}[1]
% \Procedure{$\simulateMecHeuristic ()$}{}
%     \For{$nSamples * nTransitions$ times}
%     	\State ${\action} \gets $ sampled uniformly from $\state$
%     	\State $\highlight{\tsucc} \gets$ sampled according to $\trans(\state,{\action})$
%     	\State $\highlight{\text{Increment }\#(\state,{\action},\tsucc)}$
%     	\State $\state \gets \highlight{\tsucc}$ \Comment{Move from $s$ to $t$.}
%     \EndFor
% \EndProcedure
% \end{algorithmic}
% \end{algorithm}

% In Algorithm \ref{alg:updateMEC}, the estimated mean-payoff is $\beta$-close to the actual mean payoff with probability $\ge 1-\delta$. This requires that all the estimated transition probabilities are $\epsilon$ close to the actual transition probabilities with probability $\ge 1-\delta$.


% \begin{algorithm}[H]
%     \caption{Value Iteration algorithm for blackbox MECs}\label{alg:vi}
% 		\hspace*{\algorithmicindent}\algorithmicrequire	MEC $M_i = (T_i, A_i)$, precision $\beta > 0$. \Comment{\track{Specify some requirement from input model to achieve required precision}} \\
% 		\hspace*{\algorithmicindent}\algorithmicensure mean-payoff lower bound $w_l$, mean-payoff upper bound $w_u$
% 	\begin{algorithmic}[1]
% 	    \Procedure{$\mathsf{VALUE\_ITERATION}$}{$M_i, \beta$}
% 	    \State $l_0(\cdot) \gets 0, u_0(\cdot) \gets 0, n \gets 0$
% 		\Repeat
% 		    \State $n \gets n+1$
% 		    \For{$\state \in T_i$}
% 		        \State $l_n(\state) = \max\limits_{{\action}\in\av(\state)}(r(\state, {\action}) + \widehat{\lb}(\state, {\action}))$
% 		        \State $u_n(\state) = \max\limits_{{\action}\in\av(\state)}(r(\state, {\action}) + \widehat{\ub}(\state, {\action}))$
% 		    \EndFor
% 		\Until{sp$(\Delta^{\ub}_n) > \beta$ and sp$(\Delta^{\lb}_n) > \beta$}
% 	    \State $\state \gets $ random state in $T_i$\\
% 		\Return $\max\limits_{\state\in T_i}(l_n(\state)-l_{n-1}(\state)), \max\limits_{\state\in T_i}(u_n(\state)-u_{n-1}(\state))$
% 		\EndProcedure
% 	\end{algorithmic}
% \end{algorithm}

% \begin{algorithm}[htbp]
% 	\caption{New update procedure using the probability estimates}\label{alg:updateNew}
% 			\hspace*{\algorithmicindent}\algorithmicrequire	Set of States $S$.
% 	\begin{algorithmic}[1]
% 		\Procedure{$\UPDATE$}{Set of states $S$}
% 		\For {$\state\in S$}
%     		\For {$f \in \set{\lb,\ub}$}  ~~~~~~\Comment{For both functions}
%         		\State 
%     			$ f(\state) = \max_{{\action} \in \Av(\state)} \highlight{\widehat{f}}(\state,{\action})$
%         	\EndFor
%         \EndFor
% 		\EndProcedure
% 	\end{algorithmic}
% \end{algorithm}


% \begin{algorithm}[H]
%     \caption{Deflate algorithm}\label{alg:deflate}
%         \hspace*{\algorithmicindent}\algorithmicrequire MEC $M_i = (T_i, A_i)$
%     \begin{algorithmic}[1]
%         \Procedure{$\mathsf{DEFLATE}$}{MEC $M_i$}
%             \For{$\state \in T_i$}
%                 \State $\ub(\state) = \min(\ub(\state), \widehat{\ub}(\mathsf{BEST\_LEAVING\_ACTION}(M_i)))$
%             \EndFor
%         \EndProcedure
%     \end{algorithmic}
% \end{algorithm}

\end{comment}

% This algorithm is largely an amalgamation of the CAV'17 and CAV'19 algorithms. The CAV'17 gives a framework to reduce a mean-payoff problem to a reachability problem, whereas the CAV'19 paper gives us the reachability algorithm for blackbox models. Thus, we get a mean-payoff algorithm for blackbox models.

\paragraph{Using greybox update equations during blackbox learning}
We also consider the variant where we use greybox update equations to estimate the mean-payoff values.
% However, assuming we keep the confidence width unchanged, this increases the error tolerance which now includes the probability of missing some successor of a state $s$ for an action $a$, given the number of times action $a$ has been visited from $s$\footnote{Assuming $\#(s,a)$ to be as small as $200$, and $\pmin=0.05$, the probability of missing a transition is $3.5 \cdot 10^{-5}$.}.
However, assuming we keep the confidence width unchanged, the error tolerance now has to include the probability of missing some successor of a state $s$ for an action $a$\footnote{Assuming $\#(s,a)$ to be as small as $200$, and $\pmin=0.05$, the probability of missing a transition is $3.5 \cdot 10^{-5}$.}.
%
% Below we give an example of the effect of error tolerance and confidence width due to the use of greybox Bellman update equations.
% For all benchmarks, if we keep the confidence width unchanged, thereby increasing the error tolerance, the convergence was found to be much faster than using the first type of Bellman update equations, and the value was found to be correct in all cases.
% In fact the precision is met for all benchmarks apart from \texttt{phil-nofair3}, and \texttt{rabin3} and the upper and the lower values converge within a few seconds to a few minutes.
%
% \paragraph{Effect on confidence width and error tolerance}
% We discuss the effect on confidence width and error tolerance as a result of using the greybox update equations in blackbox learning.
Given an error tolerance $\delta_{\mathbb{T}}$, and number of samples $\#(s,a)$, the probability that we miss a particular successor is at most $(1-{\pmin})^{\#(s, a)}$, and hence the error tolerance corresponding to using the greybox equations for blackbox learning increases to $\delta_{\mathbb{T}} + (1-{\pmin})^{\#(s, a)}$\footnote{This is an approximation as we only consider the error tolerance of missing one particular transition. At the same time, in an actual MDP, transition probabilities for most actions may be higher than $\pmin$ and thus, the probability of missing any transition for such actions may be lower.
%On the other hand, in an actual MDP, most transitions to successor states of $s$ under action $a$ may have probabilities that are much higher than ${\pmin}$.
}.
% Given an error tolerance $\delta_{\mathbb{T}}$, and number of samples $\#(s,a)$ (number of times a state-action pair is visited), we can obtain a confidence width $c$ using Hoeffding's inequality (See \cite{AKW19} for details) such that $\widehat{\mathbb{T}}(s, a, \tsucc) := \max (0, \dfrac{\#(s, a, t)}{\#(s, a)} - c)$.
% Assuming a minimum transition probability of ${\sf \pmin}$, the probability that we miss a particular successor is at most $(1-{\pmin})^{\#(s, a)}$, and hence the error tolerance corresponding to using the greybox equations increases to $\delta_{\mathbb{T}} + (1-{\pmin})^{\#(s, a)}$ if we use greybox equations in blackbox learning \footnote{This is an approximation since we consider the error tolerance of missing one particular transition. On the other hand, in an actual MDP, all the transitions to successor states of $s$ under action $\action$ may have probabilities that are much higher than ${\pmin}$.}.

On the other hand, if we fix the error probability $\delta_{\mathbb{T}}$ \emph{a priori}, we have, $\delta_{\mathbb{T}} = \delta'_{\mathbb{T}} + (1- \pmin)^{\#(s, a)}$\todo{redo sentence after tp-confidence, define $\delta'_{\mathbb{T}}$}, then the confidence width would increase to a new value $c' = \sqrt{\frac{\ln (\delta'_{\mathbb{T}})}{-2 \#(s, a)}}$. Note that the number of samples here remains the same.
An example showing the dependence of confidence width on error tolerance has been shown in Appendix~\ref{app:error_tolerance}.

% To the best of our knowledge, Theorem~\ref{thm:algo} gives a correctness guarantee on the first practical algorithm for blackbox learning for mean-payoff objectives on MDPs.
We also note that the use of greybox update equations on estimating the transition probabilities also gives us a PAC guarantee but with an increased error tolerance.

\paragraph{Greybox learning}
In the greybox setting, for every state-action pair $(s,a)$, we additionally know the exact number of successors $\abs{\post(s,a)}$.
% Here we sample every state-action pair until we have seen all successors.\todo{What does it mean?}
This gives an improved EC-detection mechanism.
In blackbox EC-detection, while detecting $\deltasure$-EC, we try to have many samples of the same action so that the probability that a transition might have been missed would be reduced. In greybox, on the other hand, we know the exact number of transitions for every state-action pair, and thus usually we don't need many samples to make sure that there aren't any unseen transitions.

%By the qualitative information, we immediately know if there are further transitions for a state-action pair and hence can speed up the process.
Further, we use the greybox Bellman update equations for estimating the mean-payoff values corresponding to state-action pairs where all the successors are visited, while if all the successors are not visited, we use blackbox update equations. These improvements have considerable impact on performance as demonstrated in Section~\ref{app:greybox}.

\begin{comment}

\subsection{Regarding extra sampling in Value Iteration procedure}
Since, we are now using an estimate for the probabilities of transitions, we can't simply use the standard value iteration algorithm (Algorithm 1 of CAV'17) to update the values of ECs. We have to incorporate the confidence widths for the values of the actions. This further gives rise to the need for maintaining upper and lower bounds for the values of the states in the MECs. Thus, we use a bounded value iteration algorithm (Algorithm \ref{alg:updateMEC}). Note that every call to Algorithm \ref{alg:vi} corresponds to a fixed value of confidence width $c$. Thus, we try to converge the respective upper and lower bounds of the overall MEC. The difference between the bounds would only go down if we simulate the actions of the MEC a large number of times to reduce the confidence width. Thus, before running the value iteration algorithm as in CAV'17, we simulate the MEC a large number of times (lines 1-4 in Algorithm \ref{alg:vi}).


\subsection{When to update an MEC}
The CAV'17 paper advises running value iteration on an MEC only when the simulation ends up in the $s_?$ state. However, we think that it is fine to run VI even when we reach $s_+$. CAV'17 posits that if a simulation ends up in $s_?$, it means that the gap between the upper and lower bound is quite large and hence, needs to be reduced by running VI. But we feel that it is fine to run VI even if the simulation ends up in $s_+$ because this shows that the reward lower bound of the MEC is high and it may be fruitful to run VI on this MEC and get a more precise value. This leads to a much faster convergence even in whitebox models. In the earlier case, the more number of times VI was run, the upper and lower bounds became tighter, the probability of going to $s_?$ became smaller and running VI again became very rare. Thus, achieving the required precision took a lot of simulations.


\subsection{Error tolerance}
We say from CAV'19 that $\delta_{\trans} = \dfrac{\delta\cdot \pmin}{\lvert\{{\action} \vert\, \state \in \widehat{S} \wedge {\action} \in \av(\state) \}\rvert}$. Here the maximum number of successors per action of the model is given by $\frac{1}{\pmin}$. But in many of the models, maximum number of successors  are usually less than $\frac{1}{p_{min}}$. So instead of using $\pmin$, we use the maximum number of successors while computing $\transdelta$. Then, $\delta_{\trans} = \dfrac{\delta}{\lvert\{{\action} \vert\, \state \in \widehat{S} \wedge {\action} \in \av(\state) \}\rvert \cdot maxSuccessors}$.


For zeroconf\_rewards model, we have $\pmin=0.002$ and $maxSuccessors=6$. By using the $\pmin$ we get $\transdelta$ to be approximately $3*10^{-8}$. Whereas by using the $maxSuccessors$ we get $\transdelta$ to be approximately $2*10^{-5}$. Lets assume that we have visited a state-action pair $10^7$ times. Then the confidence width using the first value of $\transdelta$ is $0.0027$ and using the second value of $\transdelta$, we get the confidence width to be $0.0021$. We get a slight improvement in confidence width, when using $maxSuccessors$ instead of $\frac{1}{\pmin}$.

\end{comment}


==> algo_ctmdp.tex <==
% As mentioned earlier, our algorithm for computing mean-payoff in blackbox CTMDPs uses the same framework we use in Section~\ref{sec:algo} for computing mean-payoff in blackbox MDPs. We compute values of the end components and we compute the probability of reaching those end components from the initial states. 
% As mentioned in \_ computing unbounded reachability probability in a CTMDP is the same as computing unbounded reachability probability in the embedded MDP. Thus, by estimating $\Delta(s,a,t)$, for all $s, a, t$ in a CTMDP, we can compute the probability of reaching end components using the same method as outlined in Section~\ref{sec:algo}. Further, we have described a method for estimating the reward values of end components in CTMDPs. Finally, our algorithm for computing mean-payoff in blackbox CTMDPs follows the outline of Algorithm~\ref{alg:general}.
% The detailed pseudocodes are provided in Appendix~\ref{app:ctmdp_algo}. \track{Merge with first para in Section 6.}

% The flow to various function calls is similar to that of learning blackbox MDP.
% % Now we describe the algorithms for blackbox learning of CTMDPs.
% We use an {\sf ON\_DEMAND\_BVI} algorithm similar to that of MDP.
% The differences are that it calls procedures $\SIMULATE{\sf \_CTMDP}$ and $\mathsf{UPDATE\_MEC\_VALUE\_CTMDP}$ instead of calling the $\SIMULATE$ and $\mathsf{UPDATE\_MEC\_VALUE}$ procedures respectively as done in the case of the algorithm for MDP.\todo{Do not use the names.}
% While simulating the CTMDP, we also estimate the rates of the state-action pairs which was not required in the case of MDPs.
% The detailed pseudocodes are provided in Appendix~\ref{app:ctmdp_algo}.

\begin{comment}

The procedure $\SIMULATE{\sf \_CTMDP}$ algorithm differs from the $\SIMULATE$ algorithm of MDP in the way that the former simulates a CTMDP, and hence when it reaches a state $\state$, and the next action $\action$ is chosen, a real time $\tau$ is also chosen following the exponential distribution with rate $\lambda(\state, \action)$.

In the procedure $\mathsf{UPDATE\_MEC\_VALUE}{\sf \_CTMDP}$, for a given input MEC, for every state-action pair $(\state, \action)$, we estimate the rate $\lambda(\state, \action)$ by simulating the MEC, and also uniformize it before calling value iteration.
This is actually done in the $\SIMULATE{\sf \_MEC}$ procedure.
Note that unlike the case of MDP where we have a single $\SIMULATE$ procedure, in CTMDP, we use two different procedures: $\SIMULATE{\sf \_CTMDP}$, and $\SIMULATE{\sf \_MEC}$.
While $\SIMULATE{\sf \_CTMDP}$ is used to simulate the CTMDP, the procedure $\SIMULATE{\sf \_MEC}$ is used to simulate a MEC in particular.
In $\SIMULATE{\sf \_MEC}$, we estimate the rates of the state-action pairs.
However, estimating the rates is not required outside the MECs. 
Hence in $\SIMULATE{\sf \_CTMDP}$, we do not estimate the rates for the states and the actions that are visited.

\end{comment}


==> deflate.tex <==
We compute the stay action (Line 12) and the corresponding probabilities for an MEC M1.
Once we have a stay action, then we treat it as a reachability problem.
Then when reinitialise the values in Line 14, where the values correspond to reachability values, we initialize upper and lower values of all states to 1 and 0 respectively.
Now it may be possible that there is an outgoing action to another MEC, say M2 with a higher mean-payoff, and we need to deflate the values of the states of M1 to the value of M2. 
Considering reachability, if the upper value is initialized to 1 for all states in M1, then the actual mean-payoff coming from MEC M2 is never properly back propagated as the upper value of all states in M1 will remain as 1 while back propagating the reachability value inside M1 as we will consider the actions within M1 while back propagating.
There is always an action from a state to a successor which is within the MEC and such that the successor has a value of 1.
Had we collapsed M1, then we would not be considering the actions within the MEC M1.
Since in the blackbox model, we are unable to collapse, we need to perform the deflate operation so that the value of MEC M2 is back propagated properly.
The deflate action lowers the upper reachability value to the best outgoing action.
Q: When can the value of U(s) go below the best\_leaving\_action? Why don't we update it to the best leaving action?

This is because collapsing would prevent us from visiting those states again, which is undesirable in a blackbox setting. However, this leads to other problems.
Consider an MDP that only has a single MEC $M$ and one outgoing action from every individual state.
Say these outgoing actions have the same distribution and reach a goal state with probability $p$.
Clearly, the reachability value of this MDP is $p$.
Now, when we do BVI to calculate this value, from every state in $M$, there would be at least 2 action choices, one that stays inside the MEC, and one that goes towards the goal state.
Initially, all states, except the terminal states would have upper and lower values set to 0 and 1, respectively.
Thus, among the 2 action choices, one would have upper value $p$, while the other would have upper value 1, and hence, the bellman update resets the upper value of the state to 1.
As one can see, this would go on, and convergence wouldn't happen.
To avoid this, we need the deflate operation which lowers the upper reachability value to the best outgoing action, i.e. in this case, the action with value $p$.
More technical details are provided in Appendix~\ref{app:algo}.

==> lp.tex <==
We first describe how to compute the mean payoff in the case of a Markov chain where all the probabilities are known.
Consider a BSCC $B$ in a Markov chain.
Insider a BSCC, we first compute the steady state distributions for each state in the BSCC.
Let $d_s$ denote the steady state distribution for each state $s$ in $B$.
For a state $s_i$, we have that $d_{s_i} = \displaystyle{\sum_{s \to s_i}}d_s \cdot p(s,s_i)$.
Then we compute the \emph{one-step expected reward} from $s$ as $e(s)=\displaystyle{\sum_{s_i \: : \: s \to s_i}} r(s,s_i) \cdot p(s,s_i)$.
Here $r(s,s_i)$ and $p(s,s_i)$ respectively denote the reward and the probability on the edge $(s,s_i)$.
Finally the mean payoff in the BSCC is computed as $\displaystyle{\sum_{s \in B}} d_s \cdot e_s$.

We write the following LP from \cite{BBCFK14} for a solution to maximization of expected mean payoff.
A solution to the LP denotes the existence of a witness strategy that maximizes the expected payoff.
All the variables assume non-negative values.

Let $r_a$ be the reward for action $a$. 
All the actions are unique.
For a state $s \in S$, we denote by $Act(s)$, the set of actions that are enabled from $s$.
For $s \neq s'$, we have that $Act(s) \cap Act(s') = \emptyset$.
For every MDP, we can have the above property without loss of generality by renaming of actions.
The objective function is to maximize the expected reward
\begin{center}
    $\displaystyle{\sum_{a \in A} x_a \cdot r_a }$
\end{center}
subject to for all $s \in S$:
\begin{enumerate}
    \item Transient flow:
    $\mathbbm{1}_{s_0}(s) + \displaystyle{\sum_{a \in A}} y_a \cdot \delta(a)(s) = y_s + \displaystyle{\sum_{a \in Act(s)}} y_a$.
    \item Recurrent flow:
    $\displaystyle{\sum_{a \in A}} x_a \cdot \delta(a)(s) = \displaystyle{\sum_{a \in Act(s)}} x_a$.
\end{enumerate}
\todo{Check constraints}
Here $x_a$ is the expected frequency of using $a$ in the long run in the recurrent behaviour.
Before the recurrent behaviour is reached in an MEC, there is the transient behaviour until an MEC is reached.
Variables $y_a$ denote the expected number of using $a$ until we switch to the recurrent behaviour, and $y_s$ denotes the probability of switching.

When we do not know the probabilities of the MDP exactly, we get their estimate by sampling. BRTDP gives an upper and a lower bound for the transition probability on each edge.
Let these bounds be denoted by $\delta^u(a)(s)$ and $\delta^l(a)(s)$ respectively.
Thus we replace $\delta(a)(s)$ with the variable $z(a)(s)$ in the LP, and add the additional inequalities $\delta^l(a)(s) \le z(a)(s) \le \delta^u(a)(s)$.
Note that using the variable $z(a)(s)$ instead of the actual probability $\delta(a)(s)$ renders the LP into a quadratic program.
